Bridging the Gap Between Learning in Discrete and Continuous Environments for Vision-and-Language Navigation

Most existing works in vision-and-language navigation (VLN) focus on either discrete or continuous environments, training agents that cannot generalize across the two. The fundamental difference between the two setups is that discrete navigation assumes prior knowledge of the connectivity graph of the environment, so that the agent can effectively transfer the problem of navigation with low-level controls to jumping from node to node with high-level actions by grounding to an image of a navigable direction. To bridge the discrete-to-continuous gap, we propose a predictor to generate a set of candidate waypoints during navigation, so that agents designed with high-level actions can be transferred to and trained in continuous environments. We refine the connectivity graph of Matterport3D to fit the continuous Habitat-Matterport3D, and train the waypoints predictor with the refined graphs to produce accessible waypoints at each time step. Moreover, we demonstrate that the predicted waypoints can be augmented during training to diversify the views and paths, and therefore enhance agent's generalization ability. Through extensive experiments we show that agents navigating in continuous environments with predicted waypoints perform significantly better than agents using low-level actions, which reduces the absolute discrete-to-continuous gap by 11.76% Success Weighted by Path Length (SPL) for the Cross-Modal Matching Agent and 18.24% SPL for the Recurrent VLN-BERT. Our agents, trained with a simple imitation learning objective, outperform previous methods by a large margin, achieving new state-of-the-art results on the testing environments of the R2R-CE and the RxR-CE datasets.

==> sections/x_temp.tex <==
% \section{Temp Tables} 
% \label{sec:temp_tables}




% % % Table 3 ---------------------------------------
% \begin{table}[t]
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|l|c|cccc|cccc}
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#}} & \multicolumn{1}{c|}{\multirow{2}{*}{Dist}} & \multicolumn{4}{c|}{R2R-CE Val-Seen} & \multicolumn{4}{c}{R2R-CE Val-Unseen}\Tstrut\\
%     \cline{4-11} &  &  & 
%     \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} &  \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$}\Tstrut\\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{3}{*}{CMA}} 
%     & 1 & 0.25 &  &  &  &  & 7.01 & 20.51 & 20.48 & 49.17 \\
%     & 2 & 1.00 &  &  &  &  &  &   \\
%     & 3 & 2.00 &  &  &  &  & 6.96 & 33.05 & 32.79 & 48.52 \\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{3}{*}{\vlnbert}} 
%     & 1 & 0.25 &  &  &  &  &  &   \\
%     & 2 & 1.00 &  &  &  &  &  &   \\
%     & 3 & 2.00 &  &  &  &  &  &   \\
%     \hline \hline
%     \end{tabular}}
%     \end{center}
%     \caption{Navigation results using waypoints at fixed directions and distances. \textit{Dist} means the forward distance (meters) in selected direction.}
%     \label{tab:fix_waypoint}
%     % \vspace{-10pt}
% \end{table}


% % Table 3+ ---------------------------------------
% \begin{table}[t]
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|l|c|cccc|cccc}
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#}} & \multicolumn{1}{c|}{\multirow{2}{*}{Dist}} & \multicolumn{4}{c|}{R2R-CE Val-Seen} & \multicolumn{4}{c}{R2R-CE Val-Unseen}\Tstrut\\
%     \cline{4-11} &  &  & 
%     \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} &  \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$}\Tstrut\\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{4}{*}{REVERIE}} 
%     & 1 & 0.25 &  &  &  &  &  &  &  &   \\
%     & 2 & 1.00 &  &  &  &  &  &  &  &   \\
%     & 3 & 2.00 &  &  &  &  &  &  &  &   \\
%     & 4 & 3.00 &  &  &  &  &  &  &  &   \\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{4}{*}{R2R}} 
%     & 1 & 0.25 &  &  &  &  & 7.01 & 20.51 & 20.48 & 49.17  \\
%     & 2 & 1.00 &  &  &  &  &  &  &  &   \\
%     & 3 & 2.00 &  &  &  &  & 6.96 & 33.05 & 32.79 & 48.52 \\
%     & 4 & 3.00 &  &  &  &  &  &  &  &   \\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{4}{*}{RxR}} 
%     & 1 & 0.25 &  &  &  &  &  &  &  &  \\
%     & 2 & 1.00 &  &  &  &  &  &  &  &  \\
%     & 3 & 2.00 &  &  &  &  &  &  &  &   \\
%     & 4 & 3.00 &  &  &  &  &  &  &  &   \\
%     \hline \hline
%     \end{tabular}}
%     \end{center}
%     \caption{Navigation results using waypoints at fixed directions and distances. \textit{Dist} means the forward distance (meters) in selected direction.}
%     \label{tab:fix_waypoint_plus}
%     % \vspace{-10pt}
% \end{table}


% % % Table 4 ---------------------------------------
% \begin{table}[t]
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|l|cccc|cccc}
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#}} &  \multicolumn{4}{c|}{R2R-CE Val-Seen} & \multicolumn{4}{c}{R2R-CE Val-Unseen}\Tstrut\\
%     \cline{3-10} &  &
%     \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} &  \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$}\Tstrut\\
%     \hline \hline
%     CMA      & 1 &  &  &  &  &  &  &   \\
%     \vlnbert & 2 &  &  &  &  &  &  &   \\
%     \hline \hline
%     \end{tabular}}
%     \end{center}
%     \caption{Navigation results with waypoint predictor trained on different environments.}
%     \label{tab:testset_waypoint}
%     % \vspace{-10pt}
% \end{table}


% % Table 5 ---------------------------------------
% \begin{table}[t]
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|l|cccc|cccc}
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{\#}} & \multicolumn{1}{c|}{\multirow{2}{*}{Model}} &
%     \multicolumn{4}{c|}{R2R-CE Test Unseen} & \multicolumn{4}{c}{RxR-CE Test Unseen}\Tstrut\\
%     \cline{3-10} &  &
%     \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} &  \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$}\Tstrut\\
%     \hline \hline
%     1 & CMA       &  &  &  &  &  &  &   \\
%     2 & \vlnbert  &  &  &  &  &  &  &   \\
%     -- & Others 1  &  &  &  &  &  &  &   \\
%     -- & Others 2  &  &  &  &  &  &  &   \\
%     \hline \hline
%     \end{tabular}}
%     \end{center}
%     \caption{Comparison with state-of-the-art agents on R2R-CE and RxR-CE testing splits.}
%     \label{tab:testset_waypoint}
%     % \vspace{-10pt}
% \end{table}


% % Table 6 ---------------------------------------
% \begin{table*}[t]
%   \begin{center}
%   \resizebox{1.00\textwidth}{!}{
%   \begin{tabular}{l|l|rr|rr|rrrrr|rrrrr}
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#}} & \multicolumn{2}{c|}{Train Connectivity} & \multicolumn{2}{c|}{Val Connectivity} & \multicolumn{5}{c|}{R2R-CE Val-Seen} &
%     \multicolumn{5}{c}{R2R-CE Val-Unseen} \\
%     \cline{3-16} & & 
%     \multicolumn{1}{c}{Graph} & \multicolumn{1}{c|}{Predictor} & \multicolumn{1}{c}{Graph} & \multicolumn{1}{c|}{Predictor} & \multicolumn{1}{c}{TL} & \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} & \multicolumn{1}{c}{TL} & \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$} \Tstrut\\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{5}{*}{CMA}} & 1 & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} & 10.47 & 6.51 & 39.60 & 33.95 & 54.97 \\
%     \cline{3-16}
%      & 2 & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} & 6.67 & 6.80 & 33.50 & 30.26 & 51.05 \\
%      & 3 & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} & 7.18 & 6.50 & 37.55 & 36.60 & 52.74 \\
%      & 4 & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark$\dag$}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%      \cline{3-16}
%     %  & 5 & \multicolumn{2}{c|}{\multirow{1}{*}{2 Stages*}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{Freeze}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\ 
%     %  & 6 & \multicolumn{2}{c|}{\multirow{1}{*}{3 Stages**}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{Freeze}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\     
%     %  \cline{3-16}
%      & 5 & \multicolumn{4}{c|}{\multirow{1}{*}{Low-Level Actions}}  &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} & 8.19 & 8.33 & 25.01 & 23.05 & 41.56 \\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{5}{*}{\vlnbert}} & 1 & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} & 14.34 & 5.22 & 50.71 & 40.85 & 57.31 \\
%     \cline{3-16}
%      & 2 & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} & 9.61 & 5.91 & 40.51 & 34.92 & 51.87 \\
%      & 3 & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} & 11.49 & 5.66 & 45.24 & 41.12 & 51.20 \\
%      & 4 & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark$\dag$}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%      \cline{3-16}
%     %  & 5 & \multicolumn{2}{c|}{\multirow{1}{*}{2 Stages}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{Freeze}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\ 
%     %  & 6 & \multicolumn{2}{c|}{\multirow{1}{*}{3 Stages}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{Freeze}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\     
%     %  \cline{3-16}
%      & 5 & \multicolumn{4}{c|}{\multirow{1}{*}{Low-Level Actions}}  &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{5}{*}{\parbox{2cm}{Scene-Memory}}} & 1 & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%     \cline{3-16}
%      & 2 & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%      & 3 & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%      & 4 & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark$\dag$}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{\checkmark}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%      \cline{3-16}
%     %  & 5 & \multicolumn{2}{c|}{\multirow{1}{*}{2 Stages}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{Freeze}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\ 
%     %  & 6 & \multicolumn{2}{c|}{\multirow{1}{*}{3 Stages}} & \multicolumn{1}{c|}{\multirow{1}{*}{}} & \multicolumn{1}{c|}{\multirow{1}{*}{Freeze}} &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\     
%     %  \cline{3-16}
%      & 5 & \multicolumn{4}{c|}{\multirow{1}{*}{Low-Level Actions}}  &  &  &  &  & \multicolumn{1}{c|}{\multirow{1}{*}{}} &  &  &  &  & \\
%     \hline \hline
%   \end{tabular}}
% \end{center}
% \caption{Comparison on agent performance in R2R-CE. Graph and Predictor means applying ground-truth connectivity graph and using predicted waypoints (from either freezed or fine-tuned waypoint predictors), respectively. 
% %*2 Stages: Train navigation on the GT graph and then fine-tune with predicted waypoints. **3 Stages: Based on 2 Stages, fine-tune the waypoint predictor with navigation.
% }
% \label{tab:main_results_r2r}
% \end{table*}

%% Figure \ref{fig:node_adjust} provides an example of modifying nodes based on these metrics. In general case, we may don't have a position ranked highest on all three metrics, so we calculated a summed rank and choose the best position. Note that if one edge couldn't be connected well (\textit{i.e.} the geodesic distance between two sides is far larger than the straight line length), we dropped these edges.
% Another criterion is the shortest edge length shouldn't be too small since the minimal distance unit of the spatial connectivity predictor is 0.25m. 
% Step 1: We first construct an initial graph: For each MP3D node, if it doesn't appear in any R2R trajectories that could be successfully transferred in VLNCE, we directly project its MP3D position to Habitat as its initial position. If it appears, we collect all the transferred continuous trajectories in VLNCE, find the shortest point to its MP3D-projected position in each trajectory and taking an average as its initial position. The connectivity between nodes is similar to MP3D graphs'. Then we merge nodes within 0.5m. If any nodes are not navigable (which locate in obstalces), we snap it to its closest navigable position so that we construct a graph that all nodes are navigable.

% (1) The shortest edge length shouldn't be too small since the minimal distance unit of the spatial connectivity predictor (2)
% Step 2: Next we modify the unnavigable edges (which have collision/intersection with obstacles) until they are all navigable by heuristics. Specifically, we randomly pick one vertex of the edge to modify. We first search 270 positions uniformly within 0.35m as our candidate new positions. For each candidate position, we connect it with its neighbors. If there are some neighbors that it couldn't be directly connected with, we add as less nodes as possible to connect this neighbor with the candidate position indirectly. Then we expect to choose a best position among these candidates which satisfies (1) has as small distance to the initial position (2) has as less added nodes (3) has as large distance to its closest obstacles (4) has as straight indirectly-connected edges (we measure this by the ratio between length of indirectly-connected edge and distance of two vertexes). Since usually we could not find a position which ranked best on all these four metrics, we find a point that ranked all well on them.

% Step 3: After making all edges navigable, we merge the nodes same way as before. Since this could result in new unnavigable nodes and edges, we snap the unnavigable nodes and modify the unnavigable edges again. We perform step 2 and merging nodes continually until all nodes and edges after merging are navigable.

% Step 4: For each trajectory in VLNCE dataset, if we couldn't find nodes close enough (i.e. within 0.8m) to its start and end positions in the connectivity graph, we further add nodes to ensure there exists graph nodes close enough to trajectories' start and end.

% \section{Ground-Truth Trajectory}
% To get the ground-truth trajectories of VLNCE dataset in our connectivity graph, for one VLNCE's trajectory, we first find three positions with closeset geodesic distances to the start of this trajectory as candidate graph starts, and similarly find three candidate ends, so we got 3$\times$3 (start, end) combinations. Then for each combination, we find the 200-shortest paths between them in our connectivity graph as our candidate. For all the 200$\times$3$\times$3 candidate paths, we first convert them to continuous paths (we chunk each edge into several small edges about 0.25m), computing the nDTW between the ground-truth continuous trajectory in VLNCE and the converted paths, then use the path with highest nDTW as the ground-truth trajectory in our graph. We directly discard the trajectories with less than 0.92 nDTW. Finally we transfered 96\% trajectories of VLNCE. 


% \paragraph{Is the Connectivity Predictor Necessary?}
% One may argue that the results of \#M3 in Table~\ref{tab:main_results_wp} is only slightly better than \#M6 in Table~\ref{tab:fix_waypoint_plus}, however, this is because the choice of a fixed step size of 1 meter happens to be a suitable step size for traveling in the MP3D environments, whereas in practice, such length is unknown beforehand. In contrast, our connectivity predictor is trained to provide structural conditioned waypoints at specific directions and distances that are beneficial to agent's future decisions. Quantitatively, we found that there are about 15\% of steps executed by \#M6 (Table~\ref{tab:fix_waypoint_plus}) collides with obstacles, while this number is only 7\% once the connectivity predictor is introduced. 


% \subsection{Fine-Tune Connectivity Predictor}
% Agents with different policy networks are trained to behave differently during navigation, while both the ground-truth and the predicted connectivity graphs are not optimal for a specific agent. As a result, we propose to fine-tune the connectivity predictor with the navigator during training to adapts agent's decisions and provides better waypoints (Figure~\ref{fig:waypoint_rl}). Firstly, the predicted connectivity leads to a list of candidate images for the navigator to perform \textit{view selection}. Based on the navigator's decision, a patch of heatmap which produces such waypoint is extracted and sampled to obtain a new waypoint. Then, the navigator executes a sequence of controls to reach the sampled waypoint to collect rewards from the environment. With the sampling probabilities and the collected rewards, we update the connectivity predictor using REINFORCE algorithm~\cite{williams1992simple}. The rewards consist of a step-wise penalty of $-1$ to encourage an efficient navigation, as well as a $\pm3$ reward depending on whether the agent reaches the target. The overall loss function of the agent is simply the sum of the imitation learning objective of the navigator $\mathcal{L}_{IL}$ and the reinforcement learning loss of the connectivity predictor $\mathcal{L}_{RL}$, as $\mathcal{L}=\mathcal{L}_{IL}+\mathcal{L}_{RL}$. Ideally, we expect the module to preserve accurate prediction of spatial connectivity, while generating waypoints tailored for a specific agent. As shown in Table~\ref{tab:main_results_wp}, 
% \begin{table}[t]
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|cc|cccc|cccc}
%         \hline \hline
%         \multicolumn{1}{c|}{\multirow{2}{*}{\#}} & \multicolumn{2}{c|}{Action} & \multicolumn{4}{c|}{R2R-CE Val-Seen} & \multicolumn{4}{c}{R2R-CE Val-Unseen}\Tstrut\\
%         \cline{2-11} &
%         \multicolumn{1}{c}{Select} & 
%         \multicolumn{1}{c|}{Teleport} & \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} &  \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$}\Tstrut\\
%         \hline \hline
%         \textcolor{red}{1}  & \checkmark & \checkmark & 6.28 & 41.61 & 36.60 & 58.37 & 6.51 & 39.60 & 33.95 & 55.41 \\
%         \hline
%         \textcolor{red}{2}  & \checkmark &            & 5.70 & 46.31 & 43.20 & 58.25 & 6.38 & 37.72 & 35.02 & 53.40 \\
%         \textcolor{red}{3}  &            & \checkmark & 7.45 & 32.08 & 26.67 & 48.67 & 7.33 & 29.80 & 24.57 & 45.33 \\
%         \hline
%         \textcolor{red}{4}  &  &                      &7.59  & 29.40 & 27.24 & 48.71 & 8.33 & 25.01 & 23.05 & 44.93 \\ 
%         \hline \hline
%     \end{tabular}}
%     \end{center}
%     \vspace{-10pt}
%     \caption{Action in continuous environments by view selection (Select) and waypoint teleportation (Teleport) with the support of connectivity graph.}
%     \label{tab:poc_results}
%     % \vspace{-10pt}
% \end{table}

% \begin{table}[t]
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|c|c|cccc|cccc}
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{\#}} & \multicolumn{1}{c|}{\multirow{2}{*}{Select}} & \multicolumn{1}{c|}{\multirow{2}{*}{Dist}} & \multicolumn{4}{c|}{R2R-CE Val-Seen} & \multicolumn{4}{c}{R2R-CE Val-Unseen}\Tstrut\\
%     \cline{4-11} &  &  & 
%     \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} &  \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$}\Tstrut\\
%     \hline \hline
%     \textcolor{red}{1} &  & 0.25 & 7.59 & 29.40 & 27.24 & 48.71 & 8.33 & 25.01 & 23.05 & 44.93  \\
%     \textcolor{red}{2} &  & 1.00 & 7.75 & 25.77 & 23.99 & 49.57 & 7.97 & 23.59 & 21.32 & 47.05  \\
%     3 &  & 2.00 &  &  &  &  & 7.79 & 21.31 & 20.01 & 46.92  \\
%     4 &  & 3.00 &  &  &  &  & 8.18 & 20.00 & 17.77 & 45.09  \\
%     \hline \hline
%     5 & \checkmark & 0.25 &  &  &  &  & 6.52 & 32.82 & 32.36 & 52.76  \\
%     \textcolor{red}{6} & \checkmark & 1.00 &  &  &  &  & 6.85 & 35.04 & 33.73 & 52.44 \\
%     7 & \checkmark & 2.00 &  &  &  &  & 6.96 & 33.05 & 32.79 & 48.52 \\
%     8 & \checkmark & 3.00 &  &  &  &  & 7.00 & 31.11 & 30.96 & 45.36  \\
%     \hline \hline
%     \end{tabular}}
%     \end{center}
%     \vspace{-10pt}
%     \caption{Navigation results using different forward distances without the connectivity graph. \textit{Dist} means the forward distance (meters) in selected direction.}
%     \label{tab:fix_waypoint_plus}
%     % \vspace{-10pt}
% \end{table}

% \begin{table}[t]
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|c|c|cccc|cccc}
%     \hline \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{\#}} & \multicolumn{1}{c|}{\multirow{2}{*}{Select}} & \multicolumn{1}{c|}{\multirow{2}{*}{Dist}} & \multicolumn{4}{c|}{R2R-CE Val-Seen} & \multicolumn{4}{c}{R2R-CE Val-Unseen}\Tstrut\\
%     \cline{4-11} &  &  & 
%     \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c|}{nDTW$\uparrow$} &  \multicolumn{1}{c}{NE$\downarrow$} & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{nDTW$\uparrow$}\Tstrut\\
%     \hline \hline
%     \textcolor{red}{1} &  & 0.25 & 7.59 & 29.40 & 27.24 & 48.71 & 8.33 & 25.01 & 23.05 & 44.93  \\
%     \textcolor{red}{2} &  & 1.00 & 7.75 & 25.77 & 23.99 & 49.57 & 7.97 & 23.59 & 21.32 & 47.05  \\
%     3 &  & 2.00 &  &  &  &  & 7.79 & 21.31 & 20.01 & 46.92  \\
%     4 &  & 3.00 &  &  &  &  & 8.18 & 20.00 & 17.77 & 45.09  \\
%     \hline \hline
%     5 & \checkmark & 0.25 &  &  &  &  & 6.52 & 32.82 & 32.36 & 52.76  \\
%     \textcolor{red}{6} & \checkmark & 1.00 &  &  &  &  & 6.85 & 35.04 & 33.73 & 52.44 \\
%     7 & \checkmark & 2.00 &  &  &  &  & 6.96 & 33.05 & 32.79 & 48.52 \\
%     8 & \checkmark & 3.00 &  &  &  &  & 7.00 & 31.11 & 30.96 & 45.36  \\
%     \hline \hline
%     \end{tabular}}
%     \end{center}
%     \vspace{-10pt}
%     \caption{Navigation results using different forward distances without the connectivity graph. \textit{Dist} means the forward distance (meters) in selected direction.}
%     \label{tab:fix_waypoint_plus}
%     % \vspace{-10pt}
% \end{table}

